Spend Classification Without Leakage: An Evaluation Harness and What It Changed in a Deployed System

Assigning a standard commodity code to a free-text purchase line underpins enterprise spend analytics, and its reported accuracy cannot be checked. Published results use proprietary data or private samples under undocumented protocols; no two compare and there is no public benchmark. We build a harness with four protocols over 1.26 million labelled purchase lines from two US state governments. Enterprises rebuy continuously, so random splits put matching item text on both sides: 60.7% and 61.2% of test rows, 54.7% and 60.6% byte for byte. On California orders the best classical baseline scores 56.0% on repeated text but 31.9% on novel text, a 24-point gap widening with taxonomy depth. Embedding retrieval shrinks the gap from 23.8 to 19.1 points; a fine-tuned transformer does not escape it. On one corpus leaky evaluation cannot separate retrieval from the transformer, while three leak-free protocols put the transformer 2.3 to 3.6 points ahead, so leaky splits hide real differences, not just flatter both. We derive an upper bound on text-only classifiers from identical text with conflicting codes: 79.4% commodity accuracy on one corpus against 98.4% on the other, so accuracy does not compare across datasets. Spend-weighting the bound reflects the amount field more than labels. In a deployment of 920,927 lines, reviewers accepted 32.4% of suggestions on the novel-text population; 29.7-35.2% brackets benchmark rates near 31.9% and 34.8%. We release the harness in production use.

==> arxivmode.tex <==
% This file is a marker, not an input. Its presence is what selects the arXiv table
% layout, in which every table is placed beside the text that cites it; see the
% build-mode note in the preamble of main.tex. The IAAI-27 layout, which collects the
% tables in the appendix to hold the body inside six pages, is simply the absence of
% this file, so neither build requires editing a switch by hand.
%
% Deleting this file from the bundle turns the appendix layout back on. Nothing reads
% what is written here.

